Spectral stability of inviscid columnar vortices

Columnar vortices are stationary solutions of the three-dimensional Euler equations with axial symmetry, where the velocity field only depends on the distance to the axis and has no component in the axial direction. Stability of such flows was first investigated by Lord Kelvin in 1880, but despite a long history the only analytical results available so far provide necessary conditions for instability under either planar or axisymmetric perturbations. The purpose of this paper is to show that columnar vortices are spectrally stable with respect to three-dimensional perturbations with no particular symmetry. Our result applies to a large family of velocity profiles, including the most common models in atmospheric flows and engineering applications. The proof is based on a homotopy argument, which allows us to concentrate in the spectral analysis of the linearized operator to a small neighborhood of the imaginary axis, where unstable eigenvalues can be excluded using integral identities and a careful study of the so-called critical layers.

==> fig1.tex <==
%paperxsize: 9.50
%paperysize: 11.00
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point      -0.8        1.05 {$0$}
\point      -0.8        4.45 {$1$}
\point       5.0        1.05 {$r$}
\point       0.45       1.05 {$\bar r$}
\point       0.2        3.35 {$\Omega(r)$}
\point       13.0       1.75 {$|a|$}
\point       6.9        6.05 {$b$}
\point       6.3        2.35 {$\bar b$}
\point       3.9        5.15 {\small Kelvin modes $\to$}
\point       3.2        3.80 {\small essential spectrum $\to$}
\point       7.2        5.15 {\small no spectrum due to \eqref{eq:HG1}}
\point       7.2        0.65 {\small no spectrum due to \eqref{eq:HG0im}}
\point       11.3       1.90 {\rotatebox{90}{\small no spectrum as}}
\point       11.9       1.85 {\rotatebox{90}{\small $L_{m,k}$ is bounded}}
\point       8.0        2.90 {\footnotesize $\leftarrow$ hypothetical}
\point       8.0        2.50 {\footnotesize unstable modes}
}}

